Structured Pruning Learns Compact and Accurate Models

The growing size of neural language models has led to increased attention in model compression. The two predominant approaches are pruning, which gradually removes weights from a pre-trained model, and distillation, which trains a smaller compact model to match a larger one. Pruning methods can significantly reduce the model size but hardly achieve large speedups as distillation. However, distillation methods require large amounts of unlabeled data and are expensive to train. In this work, we propose a task-specific structured pruning method CoFi (Coarse- and Fine-grained Pruning), which delivers highly parallelizable subnetworks and matches the distillation methods in both accuracy and latency, without resorting to any unlabeled data. Our key insight is to jointly prune coarse-grained (e.g., layers) and fine-grained (e.g., heads and hidden units) modules, which controls the pruning decision of each parameter with masks of different granularity. We also devise a layerwise distillation strategy to transfer knowledge from unpruned to pruned models during optimization. Our experiments on GLUE and SQuAD datasets show that CoFi yields models with over 10x speedups with a small accuracy drop, showing its effectiveness and efficiency compared to previous pruning and distillation approaches.

==> tables/bert_config.tex <==
%!TEX root = ../main.tex

\begin{table}[!t]
    \centering
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{lr}
    \toprule
    {Embeddings} & {23.8M (22\%)} \\
    \tableindent token/pos/seg. & $(30522 + 512 + 2) \times 768$ \\
    \midrule
    {Self-attention} ($\times 12$) & {28.3M (26\%)} \\
    \tableindent query/key: $W_K, W_Q$ & $768 \times 768, 768 \times 768$\\
    \tableindent value/att. output: $W_V, W_O$ & $768 \times 768, 768 \times 768$ \\
    \midrule
    {Feed-forward}   ($\times 12$) & {56.6M (52\%)} \\
    \tableindent up projection: $W_U$ & 768 $\times$ 3,072 \\
    \tableindent down projection: $W_D$ & 3,072 $\times$ 768 \\
    \bottomrule
    \end{tabular}
    }
    \caption{The \# of parameters in BERT$_{\text{base}}$ model (total: 110M). A BERT model consists of embeddings and $L$ Transformer blocks, each consisting of a multi-head self-attention layer and a feed-forward layer. \danqi{This table probably needs to be out.}}
    \label{tab:bert_config}
\end{table}


==> tables/sparsity95_results.tex <==
%!TEX root = ../main.tex

\begin{table*}[t]
\resizebox{2.0\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccccccccc@{}}
\toprule
& \multicolumn{2}{c}{no layer pruning}          & \multicolumn{8}{c}{layer pruning}                                                                                         & \multicolumn{2}{c}{TinyBERT4}        &    \multicolumn{2}{c}{}         \\ \cmidrule(l{2pt}r{2pt}){2-3} \cmidrule(l{2pt}r{2pt}){4-11} \cmidrule(l{1pt}r{1pt}){12-13} \cmidrule(l{1pt}r{1pt}){14-15}
              & \multicolumn{2}{c}{Type 3} & \multicolumn{2}{c}{Type 1} & \multicolumn{2}{c}{Type 2} & \multicolumn{2}{c}{Type 3} & \multicolumn{2}{c}{Type 1 hidden} & \multicolumn{2}{c}{Type 3} & \multicolumn{2}{c}{No Distill} \\ \cmidrule(l{2pt}r{2pt}){2-3} \cmidrule(l{2pt}r{2pt}){4-5}\cmidrule(l{2pt}r{2pt}){6-7}\cmidrule(l{2pt}r{2pt}){8-9} \cmidrule(l{1pt}r{1pt}){10-11} \cmidrule(l{1pt}r{1pt}){12-13} \cmidrule(l{1pt}r{1pt}){14-15}
SST-2         & 6.96X                  & 88.65                & 13.83X          & 89.45         & 10.88X               & 90.48             & 10.35X                & 89.79& 11.42X & 91.06                  & 11.40X                 & 89.68        & 14.81X	& 86.12
        \\
QNLI          & 7.19X                  & 84.55                & 12.71X          & 84.75         & 11.35X              & 85.78             & 10.18X                & 86.34              &   13.67X &	85.08 & 11.40X                 & 86.72       & 14.51X &	83.64         \\
MNLI          & 6.98X                  & 78.35                & 12.40X          & 78.92         & 11.35X              & 79.60             & 11.68X &  79.63  & & & 11.40X                 & 78.79                \\
QQP           & 7.20X                  & 88.68                & 11.97X          & 90.00         & 11.64X              & 89.66             & 11.49X & 89.95  & & &  11.40X                 & 90.00                \\
SQuAD         & 6.41X                  & 74.08                & 8.11X           & 82.44         &                &              &                  &    & &       & 8.69X                  & 82.20                \\ \bottomrule
\end{tabular}}

\caption{Results of pruned models of a sparsity 95\% from head and intermediate dimension pruning. \todo{Add TinyBERT4 without general distillation results to the table.} \todo{Add your layer pruning without distillation either in this table or another ablation table.}}
\label{tab:sparsity95}
\end{table*}


==> tables/tinybert_small_datasets.tex <==
\begin{table}[h]
\centering
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}\toprule
      & \multicolumn{2}{c}{{\ours}} & \multicolumn{3}{c}{TinyBERT${_4}$} \\
      & speedup          & accuracy         & speedup   & w/o GD   & w/ GD  \\ \midrule
CoLA & $11.8\times$            & $30.2_{\pm 2.6}$         & $11.4\times$     & $16.6$    & $\bf{32.5}$  \\
RTE  & $10.9\times$             & $\bf{65.1_{\pm 1.6}}$         & $11.4\times$     & $47.3$    & $63.2$  \\
STS-B  & $12.2\times$               & $83.0_{\pm 1.7}$             & $11.4\times$     & $17.8$    & $\bf{85.0}$  \\
MRPC   & $11.9\times$                & {$\bf{82.6_{\pm 0.9}}$}             & $11.4\times$     & $68.9$    & $81.4$  \\ \bottomrule
\end{tabular}}

\caption{{\ours} v.s. TinyBERT${_4}$ models on GLUE datasets of a relatively small size. w/o GD denotes that we train a TinyBERT$_4$ structure from scratch with task distillation. w/ GD denotes that we train TinyBERT$_4$ from general distillation with task distillation.}
\label{tab:tinybert_small_datasets}
\end{table}

 
